An Empirical Study of Evaluating Long-form Question Answering

\Ac{LFQA} aims to generate lengthy answers to complex questions. This scenario presents great flexibility as well as significant challenges for evaluation. Most evaluations rely on deterministic metrics that depend on string or n-gram matching, while the reliability of large language model-based evaluations for long-form answers remains relatively unexplored. We address this gap by conducting an in-depth study of long-form answer evaluation with the following research questions: (i) To what extent do existing automatic evaluation metrics serve as a substitute for human evaluations? (ii) What are the limitations of existing evaluation metrics compared to human evaluations? (iii) How can the effectiveness and robustness of existing evaluation methods be improved? We collect 5,236 factoid and non-factoid long-form answers generated by different large language models and conduct a human evaluation on 2,079 of them, focusing on correctness and informativeness. Subsequently, we investigated the performance of automatic evaluation metrics by evaluating these answers, analyzing the consistency between these metrics and human evaluations. We find that the style, length of the answers, and the category of questions can bias the automatic evaluation metrics. However, fine-grained evaluation helps mitigate this issue on some metrics. Our findings have important implications for the use of large language models for evaluating long-form question answering. All code and datasets are available at https://github.com/bugtig6351/lfqa_evaluation.

==> figures/figure-temperature-study.tex <==


\definecolor{mercury}{RGB}{240,240,240}
\definecolor{gallery}{RGB}{250,250,250}
\definecolor{free_speech_aquamarine}{RGB}{0, 156, 114}
\definecolor{shakespeare}{RGB}{35, 184, 223}
\definecolor{flamingo}{RGB}{237, 88, 85}
% \definecolor{c1}{RGB}{102, 153, 204} 
% \definecolor{c2}{RGB}{153, 204, 153} 
% \definecolor{c3}{RGB}{255, 178, 102} 
% \definecolor{c4}{RGB}{204, 153, 255} 
% \definecolor{c5}{RGB}{255, 204, 153} 
% \definecolor{c6}{RGB}{153, 153, 204} 
% \definecolor{c7}{RGB}{204, 102, 102} 
% \definecolor{c8}{RGB}{153, 204, 204} 
% \definecolor{c9}{RGB}{204, 204, 102} 
% \definecolor{c10}{RGB}{178, 178, 178}

\definecolor{c1}{RGB}{51, 102, 204} 
\definecolor{c2}{RGB}{102, 204, 102} 
\definecolor{c3}{RGB}{255, 153, 51} 
\definecolor{c4}{RGB}{153, 102, 255} 
\definecolor{c5}{RGB}{255, 178, 102} 
\definecolor{c6}{RGB}{102, 102, 204} 
\definecolor{c7}{RGB}{204, 51, 51} 
\definecolor{c8}{RGB}{102, 178, 178} 
\definecolor{c9}{RGB}{204, 178, 51} 
\definecolor{c10}{RGB}{128, 128, 128}



\pgfplotsset{
axis background/.style={fill=white},
grid=both,
  xtick pos=left,
  ytick pos=left,
  tick style={
    major grid style={style=gallery,line width=1pt},
    minor grid style=mercury,
    %draw=none
    },
  minor tick num=1,
}

% \clearpage
\begin{figure*}[t]
\centering
\pgfplotslegendfromname{sharedlegend}
\begin{tikzpicture}
  \begin{groupplot}[
    group style={
      group size=3 by 3, % 3 列 1 行
      horizontal sep=0.75cm, % 子图之间的水平间距
      vertical sep=0.75cm,   % 子图之间的垂直间距
      ylabels at=edge left
    },
    height=.32\textwidth, % 每个子图的高度
    width=.35\textwidth,  % 每个子图的宽度
    legend style={
          font=\small,
          legend columns=5,
          at={(0.5,1.02)},
          anchor=south,
          /tikz/every even column/.append style={column sep=0.9mm},
          yshift=5px
        },
    legend to name=sharedlegend,
    legend entries = {claude-3.5,gemini-2.0,gpt-4o,gpt-3.5-turbo,glm4-9b,llama3-8b,solar-10.7b,mistral-7b,llama2-13b,llama2-7b},
    ymajorgrids=true,
    axis lines=box,
    enlarge x limits=0.05,
    tickwidth=0pt,
    ylabel style={yshift=-10pt}, % 减少 ylabel 和图之间的间距
    title style={
      at={(0.5,-0.15)}, % 标题位置：X 方向居中，Y 方向放在下方
      anchor=north, % 标题的锚点
      font=\small % 标题字体大小
    }
  ]

  % 第 1 个子图
  \nextgroupplot[
    ymin=6,
    ymax=9,
    ylabel={Wikieval},
    ytick={6, 6.5, 7, 7.5, 8, 8.5, 9},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
  ]
     \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.26) (2, 8.12) (3, 8.22) (4, 8.18) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.86) (2, 7.46) (3, 7.58) (4, 7.78) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.08) (2, 7.90) (3, 8.32) (4, 8.24) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.92) (2, 8.00) (3, 7.86) (4, 7.94) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.62) (2, 8.46) (3, 8.54) (4, 8.42) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.66) (2, 7.64) (3, 7.84) (4, 7.82) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.94) (2, 8.10) (3, 8.16) (4, 8.12) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.20) (2, 8.16) (3, 8.16) (4, 7.98) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.82) (2, 6.86) (3, 6.90) (4, 7.00) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.60) (2, 6.64) (3, 6.74) (4, 6.56) 
      };

  % 第 2 个子图
  \nextgroupplot[
    ymin=5,
    ymax=8,
    ytick={5, 5.5, 6, 6.5, 7, 7.5, 8},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
  ]
  \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.40) (2, 6.28) (3, 6.38) (4, 6.32) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.72) (2, 5.74) (3, 5.76) (4, 5.70) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.22) (2, 6.22) (3, 6.32) (4, 6.26) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.90) (2, 5.74) (3, 5.78) (4, 5.72) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.92) (2, 6.76) (3, 6.86) (4, 6.80) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.14) (2, 6.12) (3, 6.00) (4, 6.54) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.52) (2, 6.56) (3, 6.54) (4, 6.70) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.74) (2, 6.90) (3, 6.78) (4, 7.42) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.64) (2, 5.62) (3, 5.46) (4, 5.40) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.54) (2, 5.38) (3, 5.36) (4, 5.76) 
      };

  % 第 3 个子图
  \nextgroupplot[
    ymin=7.5,
    ymax=10,
    ytick={7.5, 8, 8.5, 9, 9.5, 10},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
  ]
 \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.98) (2, 9.30) (3, 9.42) (4, 9.28) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.14) (2, 9.16) (3, 8.84) (4, 9.32) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.20) (2, 9.40) (3, 9.34) (4, 9.14) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.12) (2, 9.48) (3, 9.36) (4, 9.30) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.28) (2, 9.36) (3, 9.20) (4, 9.30) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.32) (2, 9.14) (3, 9.22) (4, 9.12) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.18) (2, 9.36) (3, 9.22) (4, 9.08) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.18) (2, 9.28) (3, 9.32) (4, 9.02) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.00) (2, 8.24) (3, 8.16) (4, 7.94) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.00) (2, 8.04) (3, 7.98) (4, 8.22) 
      };
      
    %4
  \nextgroupplot[
    ymin=2.5,
    ymax=9.5,
    ylabel={ANTIQUE},
    ytick={3, 4, 5, 6, 7, 8, 9},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
  ]
    \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.25) (2, 8.11) (3, 8.22) (4, 8.03) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.69) (2, 8.65) (3, 8.78) (4, 8.80) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.19) (2, 8.01) (3, 8.22) (4, 8.24) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.48) (2, 7.45) (3, 7.22) (4, 7.53) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.62) (2, 7.32) (3, 7.68) (4, 7.70) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.19) (2, 5.11) (3, 5.07) (4, 5.10) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.34) (2, 6.22) (3, 6.27) (4, 6.25) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 2.88) (2, 2.88) (3, 2.94) (4, 2.86) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.42) (2, 4.44) (3, 4.44) (4, 4.49) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.08) (2, 4.09) (3, 4.05) (4, 4.00) 
      };

    % 5
    \nextgroupplot[
    ymin=2.5,
    ymax=9.5,
    ytick={3, 4, 5, 6, 7, 8, 9},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
    ]
    \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.28) (2, 8.30) (3, 8.07) (4, 8.17) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.84) (2, 8.82) (3, 8.64) (4, 8.64) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.30) (2, 8.18) (3, 8.12) (4, 8.11) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.83) (2, 7.74) (3, 7.78) (4, 7.61) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.78) (2, 7.75) (3, 7.65) (4, 7.56) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.02) (2, 5.05) (3, 4.91) (4, 5.04) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.13) (2, 6.22) (3, 6.12) (4, 6.20) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 2.83) (2, 3.02) (3, 2.90) (4, 2.98) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.43) (2, 4.49) (3, 4.50) (4, 4.52) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.06) (2, 4.11) (3, 4.01) (4, 4.06) 
      };

    % 6
    \nextgroupplot[
    ymin=3,
    ymax=10,
    ytick={3, 4, 5, 6, 7, 8, 9, 10},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
    ]
    \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.07) (2, 9.13) (3, 9.10) (4, 9.01) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.68) (2, 9.71) (3, 9.66) (4, 9.67) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.95) (2, 8.99) (3, 8.95) (4, 8.92) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.17) (2, 8.29) (3, 8.19) (4, 8.23) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.70) (2, 8.72) (3, 8.75) (4, 8.76) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.03) (2, 6.06) (3, 6.11) (4, 5.95) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.38) (2, 7.53) (3, 7.47) (4, 7.39) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 3.29) (2, 3.30) (3, 3.21) (4, 3.25) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.32) (2, 5.40) (3, 5.42) (4, 5.34) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.77) (2, 4.74) (3, 4.71) (4, 4.75) 
      };
      

    % 7
    \nextgroupplot[
    title={GPT-4o}, % 子图标题
    ymin=2.5,
    ymax=9.5,
    ylabel={ASQA},
    ytick={3, 4, 5, 6, 7, 8, 9},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
    ]
    \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.7) (2, 8.7) (3, 8.7) (4, 8.6) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.7) (2, 6.7) (3, 6.7) (4, 6.8) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.1) (2, 8.2) (3, 8.2) (4, 8.2) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.7) (2, 4.7) (3, 4.7) (4, 4.6) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.9) (2, 4.9) (3, 4.9) (4, 4.9) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.3) (2, 4.4) (3, 4.4) (4, 4.4) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.7) (2, 4.7) (3, 4.8) (4, 4.8) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 3.0) (2, 3.1) (3, 3.0) (4, 3.0) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.0) (2, 4.0) (3, 4.1) (4, 4.0) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 3.6) (2, 3.5) (3, 3.6) (4, 3.6) 
      };

    % 8
    \nextgroupplot[
    title={Claude-3.5}, % 子图标题
    ymin=2.5,
    ymax=9.5,
    ytick={3, 4, 5, 6, 7, 8, 9},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
    ]
    \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 8.6) (2, 8.5) (3, 8.6) (4, 8.5) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.2) (2, 6.2) (3, 6.2) (4, 6.2) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.3) (2, 7.0) (3, 6.9) (4, 6.9) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.6) (2, 4.7) (3, 4.7) (4, 4.7) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.0) (2, 5.0) (3, 5.0) (4, 5.1) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.2) (2, 4.2) (3, 4.1) (4, 4.2) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.2) (2, 5.2) (3, 5.2) (4, 5.2) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 3.1) (2, 3.1) (3, 3.1) (4, 3.1) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 3.9) (2, 3.9) (3, 4.0) (4, 3.9) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 3.6) (2, 3.5) (3, 3.5) (4, 3.5) 
      };

    % 9
    \nextgroupplot[
    title={Gemini-2.0}, % 子图标题
    ymin=3.5,
    ymax=10.5,
    ytick={4, 5, 6, 7, 8, 9, 10},
    xticklabels={0.0,0.3,0.7,1.0},
    xtick={1,2,3,4}
    ]
    \addplot[color=c1, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.7) (2, 9.8) (3, 9.8) (4, 9.8) 
      };
      \addplot[color=c2, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.2) (2, 9.2) (3, 9.2) (4, 9.2) 
      };
      \addplot[color=c3, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 9.4) (2, 9.4) (3, 9.4) (4, 9.4) 
      };
      \addplot[color=c4, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.6) (2, 6.6) (3, 6.6) (4, 6.6) 
      };
      \addplot[color=c5, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.2) (2, 7.0) (3, 7.1) (4, 7.1) 
      };
      \addplot[color=c6, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 6.2) (2, 6.2) (3, 6.2) (4, 6.3) 
      };
      \addplot[color=c7, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 7.9) (2, 7.7) (3, 7.8) (4, 7.8) 
      };
      \addplot[color=c8, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.2) (2, 4.2) (3, 4.3) (4, 4.3) 
      };
      \addplot[color=c9, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 5.8) (2, 5.7) (3, 5.8) (4, 5.7) 
      };
      \addplot[color=c10, dashed, mark=*, mark options={scale=0.5, solid},thick] coordinates {
      	(1, 4.9) (2, 5.0) (3, 5.0) (4, 5.0) 
      };

  \end{groupplot} 
\end{tikzpicture}
\caption{The relationship between model average scores and evaluators' sampling temperature.}
\label{fig:temperature_lines}
\end{figure*}
% \clearpage

